BC-Z: Zero-Shot Task Generalization with Robotic Imitation Learning

In this paper, we study the problem of enabling a vision-based robotic manipulation system to generalize to novel tasks, a long-standing challenge in robot learning. We approach the challenge from an imitation learning perspective, aiming to study how scaling and broadening the data collected can facilitate such generalization. To that end, we develop an interactive and flexible imitation learning system that can learn from both demonstrations and interventions and can be conditioned on different forms of information that convey the task, including pre-trained embeddings of natural language or videos of humans performing the task. When scaling data collection on a real robot to more than 100 distinct tasks, we find that this system can perform 24 unseen manipulation tasks with an average success rate of 44%, without any robot demonstrations for those tasks.

==> LfD_CoRL (1)/21_task_results.tex <==

\begin{table}
\small
  \caption{\small Performance comparsion one-hot, language, or video conditioning over 21 training tasks. Video policies are conditioned on held-out videos of the training tasks. Tasks are ordered by increasing average ``Demo Length'', the number of states observed per expert demonstration, or roughly how many actions the learning policy must learn per episode (both executing at 10 Hz). Length is treated as an estimate of difficulty.
  %a learned policy can be expected to make (both at 10Hz).
  A subset of eight tasks denoted by \eighttask~are used for comparing additional ablations. Numbers in (parentheses) are 1 unit standard deviation. \emph{See Table~\ref{table:remainingtrainsubtasks} for remaining training tasks.}}
  \label{table:traintasks}
\begin{center}
% \begin{tabular}{p{6.5cm} p{1.5cm} p{2cm} p{2cm} p{2cm}}
\resizebox{\columnwidth}{!}{
\begin{tabular}{lp{2cm}lll}
\toprule
\textbf{Tasks From 21-Task Family} & \textbf{Demo Length} & \textbf{One-Hot} & \textbf{Language} & \textbf{Video} \\
\midrule
% results from b/186856721 evaluation
`knock the eraser over' & 54 (20) & 65\% (7.0) & 91\% (8.7) & 40\% (21.9) \\
`knock the bottle over' & 61 (22) & 58\% (7.4) & 71\% (12.1) & 83\% (15.2) \\
`pick up the ceramic cup'\eighttask & 65 (25) & 67\% (4.7) & 56\% (7.2) &  83\% (15.2) \\
`pick up the ceramic bowl' & 73 (32) & 65\% (7.3) & 77\% (11.7) & 35\% (12.8) \\
`push the ceramic bowl across the table' & 89 (42) & 67\% (8.2) & 58\% (14.2) & 50\% (35.4) \\
`place the pepper in the ceramic bowl' & 98 (30) & 33\% (6.5) & 39\% (11.5) & 12.5\% (11.7) \\
`place the ceramic cup in the ceramic bowl' & 103 (26) & 22\% (6.5) & 33\% (13.6) & 66\% (27.2) \\
`place the white sponge in the ceramic bowl'\eighttask & 106 (32) & 43\% (5.1) & 38\% (6.7) & 14\% (13.2) \\
`place the bottle in the ceramic bowl'\eighttask & 110 (32) & 45\% (5.3) & 52\% (6.3) & 43\% (18.7) \\
`drag the pepper across the table'\eighttask & 115 (43) & 55\% (5.0) & 33\% (8.2) & 20\% (12.6) \\
`push the eraser across the table'\eighttask & 117 (50) & 71\% (4.7) & 45\% (7.9) & 0\% (0) \\
`place the eraser on the white sponge'\eighttask & 121 (37) & 33\% (4.9) & 30\% (7.2) & 25\% (15.3) \\
`place the pepper on the white sponge' & 123 (44) & 36\% (7.1) & 83\% (10.8) & 0\% (0) \\
`place the pepper in the ceramic cup'\eighttask & 128 (44) & 30\% (4.6) & 49\% (7.6) & 0\% (0) \\
`place the ceramic cup over the eraser' & 130 (38)  & 9\% (5.0) & 0\% (0) & 0\% (0) \\
`place the white sponge in the ceramic cup' & 131 (38) & 21\% (6.9) & 25\% (10.8) & 14\% (13.2) \\
`place the eraser in the ceramic cup'\eighttask & 135 (43) & 37\% (4.8) & 33\% (7.5) & 20\% (17.9) \\
`move the arm in a circular motion' & 144 (69) & 69\% (6.7) & 12\% (6.8) & 0\% (0) \\
`drag the ceramic bowl in a circle' & 164 (65) & 32\% (6.8) & 0\% (0) & 0\% (0) \\
`wipe the white sponge on the table' & 177 (59) & 29\% (7.8) & 18\% (9.2) & 0\% (0) \\
`stand the bottle upright' & 186 (55) & 5\% (3.5) & 0\% (0) & 0\% (0) \\
\midrule
\textit{Overall} & 115 & 42\%& 40\% & 24\%  \\
% \\
\bottomrule
\end{tabular}
}
\end{center}
\end{table}


==> LfD_CoRL (1)/A-abstract.tex <==
\begin{abstract}
In this paper, we study the problem of enabling a vision-based robotic manipulation system to generalize to novel tasks, a long-standing challenge in robot learning. We approach the challenge from an imitation learning perspective, aiming to study how scaling and broadening the data collected can facilitate such generalization. To that end, we develop an interactive and flexible imitation learning system that can learn from both demonstrations and interventions and can be conditioned on different forms of information that convey the task, including pre-trained embeddings of natural language or videos of humans performing the task. When scaling data collection on a real robot to more than 100 distinct tasks, we find that this system can perform \numholdout \emph{unseen} manipulation tasks with an average success rate of \holdoutsuccess, without any robot demonstrations for those tasks.%\footnote{Supplementary videos can be found at \url{https://sites.google.com/view/bc0-anon}} % Our experiments further suggest that reaching the same level of performance with single-task imitation learning would require more than \todo{$100$} demonstrations of each test task.
\end{abstract}

\iffalse
    In this paper, we study the problem of enabling a vision-based robotic manipulation system to generalize across diverse scenes and diverse tasks, a long-standing challenge in robot learning. We approach the above challenge from an imitation learning perspective, aiming to study how scaling and broadening the data collected can facilitate generalization to new scenes and tasks. To that end, we develop a %shared-autonomy
    DAgger-based imitation learning system to collect expert demos and demonstrate corrective behavior via VR teleoperation, along with
    %for demonstrating correct behavior to the robot along with
    an imitation learning method that can flexibly condition on task embeddings computed from language or video to perform different tasks. Using this system, we scale data collection to dozens of scenes and over 100 tasks.
    %and investigate how various design choices translate to performance.
    Said system enables a real robot
    %using the same neural network architecture for learning policies,
    to open swing doors and latched doors it has never seen before (success rates of 94\% and 27\%), and perform at least \numholdout~unseen manipulation tasks with a success rate of \todo{50\%}.
\fi
    
     %%CF.5.16: I think it's quite important to have a few sentences of motivation. Otherwise, the reader won't know why this matters.
    %%CF.5.16: It could even be something as simple as: 
    %%CF.5.29: There is quite a disconnect between the above sentence and the below sentence. In what way does the below address the problem above? Here's an initial draft of how we could write the rest of the abstract
    %%EJ.6.1 - great, lgtm.
    %%AI.6.16 - doing another pass of below.
    
    % We develop a shared-autonomy system that provides multi-task policy evaluation concurrently with data collection for human-in-the-loop imitation learning. We apply this system to achieve zero-shot generalization to a new visuomotor tasks and scenes on a real robot, using flexible form of task conditioning that can either take as input a language command or a video of a human showing the robot what to do.
    % for learning robotic policies that map monocular RGB images directly to control using deep neural networks, and apply the same architecture to solve multiple real mobile manipulation tasks:
    %%CF.5.16: I don't think this sentence above is unique to this work. It _might_ be with mobile in there, but that's not the main point of the paper. To me, the main points of the paper is: zero-shot generalization to a new visuomotor task (and scene?) on a real robot, using flexible form of task conditioning that can either take as input a language command or a video of a human showing the robot to do. We may even want to pitch it not as a new method but as a system or framework.
    % a bin-emptying grasping task, a multi-scene door opening task, and finally, a task-conditioned policy capable of performing 104 unique manipulation tasks, including zero-shot generalization to tasks it was never trained to do. The network is trained using a novel .
    %%CF.5.16: It is very difficult for the reader to know why this is a good choice and what problem it is solving. Additional motivation/context would be helpful (and it's best to provide that motivation before stating the choice)
    % The network can be conditioned on arbitrary task embeddings, and we demonstrate zero-shot task generalization to both human language and human video demonstrations. 
    %%CF.5.16: Should describe the results more precisely once they are in. (success rate, robot used, comparisons)
    %%CF.5.16: should only use surprising if it is very obviously surprising, which I don't think is the case here.
    % effectiveness of simple behavior cloning approaches to scale to real-world, unstructured environments.

==> LfD_CoRL (1)/B-introduction.tex <==



\section{Introduction}
%%CF.5.16: Outline I would recommend (copied from email) - 
% Paragraph 1: Current motivation (which is great!) + crisp problem statement
    %%CF.5.16: I think this motivation is great.
    One of the grand challenges in robotics is to create a general-purpose robot capable of performing a multitude of tasks in unstructured environments based on arbitrary user commands.
    The key challenge in this endeavour is \emph{generalization}: the robot must handle new environments, recognize and manipulate objects it has not seen before, and understand the intent of a command it has never been asked to execute. 
    End-to-end learning from pixels is a flexible choice for modeling the behavior of such generalist robots,
    as it has minimal assumptions about the state representation of the world. With sufficient real-world data, these methods should in principle enable robots to generalize across new tasks, objects, and scenes without requiring hand-coded, task-specific representations. 
    %within the policy.
    However, realizing this goal has generally remained elusive.
    %because it allows generalization across new tasks \todo{cite}, objects \todo{cite}, and scenes \todo{cite} without relying on hand-coded, task-specific representations within the policy.
    In this paper, we study the problem of enabling a robot to generalize zero-shot \rebuttal{or few-shot} to new vision-based manipulation tasks.
    

    We study this problem using the framework of imitation learning. Prior works on imitation learning have shown one-shot or zero-shot generalization to new objects~\cite{finn2017one,james2018task,yu2018one,bonardi2020learning,young2020visual} and to new object goal configurations~\cite{duan2017one,dasari2020transformers}. However, zero-shot generalization to new tasks remains a challenge, particularly when considering vision-based manipulation tasks that cover a breadth of skills (e.g., wiping, pushing, pick-and-place) with diverse objects. Achieving such generalization depends on solving challenges relating to scaling up data collection and learning algorithms for diverse data.
    
    \begin{figure}[h]
  \centering
  \vspace{-0.1cm}
    \includegraphics[width=\textwidth]{figures/overview_v3.png} 
    %\vspace{-0.2cm}
    \caption{\small Overview of \methodname. We collect a large-scale dataset (\numrobotdemos episodes) of  100 diverse manipulation tasks, and train a 7-DoF multi-task policy that conditions on task language strings or human video. We show this system produces a policy that is capable of generalizing zero-shot to new unseen tasks.}
    % In this work we build a multi-task lifelong imitation learning system, and apply it in various task scenarios to show that end-to-end machine learning is capable of various forms of generalization: zero-shot generalization to novel object configurations in a pick-and-place task, zero-shot generalization to new doors in a door opening task, and finally, zero-shot generalization to new user specified tasks in a multi-task manipulation setting. This model can be flexibly conditioned on any contextual embedding, such as from human video and natural language.}
  \label{fig:overview}
 \vspace{-10pt}
\end{figure}
    
    \iffalse
    We study this problem using the framework of imitation learning. While imitation learning methods have been developed to rapidly adapt to new objects~\cite{finn2017one,james2018task,yu2018one,bonardi2020learning,young2020visual} or new object configurations~\cite{duan2017one,dasari2020transformers},
    %%CF: Let's leave silver2020few to the related work, since it's not doing robot manipulation.
    zero-shot generalization to new tasks remains a major challenge, particularly when considering closed-loop, 6-DoF manipulation tasks that cover a breadth of skills (e.g. grasping, wiping, pushing, pick-and-place) with diverse objects. In this work, we focus on expanding the zero-shot generalization capabilities of such end-to-end policies in manipulation tasks.
    \fi
    %%TODO(Chelsea): add more nuanced discussion of how prior works like DAML, duan, james do not solve the problem we want to solve. (i.e. we want a single policy that can generalize across a breadth of overarching skills (e.g. grasping, wiping, pick-and-place, pushing) and to new tasks zero-shot (e.g. grasping a banana and placing it into a tray on a cluttered table)
    %%CF.5.29: should try to get across that we are focusing on manipulation & mobile manipulation
    %%CF.5.29: The above seems to be lacking an explicit mention of the problem we want to solve. This will be important because when you start discussing prior works, it's important that it be clear to the reader why these prior works don't address the problem we are trying to solve. If they don't know exactly what problem we want to solve, then it definitely won't be clear :)
    %%EJ.6.1: Thanks, added some more content above.
    % Paragraph 2: Briefly discuss prior works that have shown some degree of generalization, but that zero-shot generalization to new tasks and scenes remains a major challenge. Describe why it's hard -- the need to scale up and all of the challenges associated with scaling up
    % The most impressive feats of generalization behavior to date are achieved by a combination of large-scale datasets coupled with end-to-end machine learning, typically implemented using large neural networks. 
    %%CF.5.29: It might be a good idea have a little bit of motivation for why end-to-end ML from raw pixel observations makes sense. It makes it a lot easier to generalize across tasks and objects because you don't need hand-defined, task-specific state representations, but that might not be obvious to all readers? Not sure. I do think that this sort of task specific engineering is different in robotics from what feature engineering in speech and vision looks like.
    % Consistent with a body of work showing that end-to-end learning outperforms task-specific engineering on speech, vision, and natural language domains \todo{cite works from representative citations}, prior work on end-to-end robotic learning from pixels have exhibited generalization to new scenes \todo{cite https://arxiv.org/pdf/1807.07049.pdf}, new objects \todo{cite Redmond 2014,
    %%CF.5.29: what is Redmond 2014? 
    %%EJ.6.1 one of the earlier 2D grasping papers showing new object generalization from grasping (redmond and angelova et al).
    % levine, etc}, and new tasks \todo{hausman, etc}. 
    %%CF.5.29: Missing most important part -- in what way do these prior works not address the problem we are trying to solve? (For this, I would suggest saying that zero-shot generalization to new tasks and scenes remains a major challenge, particularly for robotic manipulation, while also having a slightly more nuanced discussion of prior work.)
    % Paragraph 3: Guide the reader to how we address the challenges associated with scaling up & generalization 
    %Scaling up data diversity and model capacity are central to improving the generalization capabilities of any learning system, but there are practical challenges to solve before ``simply scaling up" can be applied to robotic imitation learning: we need a way to collect high-quality data across many tasks and a means to train models on such multi-task data in a way that supports generalization to entirely new tasks. 
    We develop an interactive imitation learning system with two key properties that enable high-quality data collection and generalization to entirely new tasks. First, our system incorporates shared autonomy into teleoperation to allow us to collect both raw demonstration data and human interventions to correct the robot's current policy. Second, our system flexibly conditions the policy on different forms of task specification, including a language instruction or a video of a person performing the task. Unlike discrete one-hot task identifiers~\cite{rahmatizadeh2018vision}, these continuous forms of task specification can in principle enable the robot to generalize zero-shot \rebuttal{or few-shot} to new tasks by providing a language or video command of the new task at test time.
    These properties have been explored previously; our aim is to empirically study whether these ideas scale to a broad range of real-world tasks.
    
    \iffalse
    Input feature and output label design is an open-ended design problem: how should action primitives be represented so that tasks can be learned efficiently, and yet flexible enough to express a wide variety of general-purpose behaviors? How should general task specification be numerically represented? How do we ensure that inputs to models contain sufficient information to predict actions for a wide variety of tasks, but not too much as to burden the learner? The very nature of training general-purpose robots, which require collecting lots of diverse data and need to be validated across diverse conditions, make these design questions hard to iterate on in the real world. 
    \fi
    %%CF.5.29: The above two paragraphs seem to be talking more about the problem and what makes it hard, rather than actually getting to what our insights are and what we do to solve the problem. If the key components of our system are the shared autonomy data collection scheme and the flexible task conditioning, then it would be good to mention those aspects (and not just stating them, but guiding the reader to those components)
    %%CF.5.29: Also, recall our conversation in the meeting about how combined data collection and evaluation probably won't register with readers because it's a few steps ahead of how people will be thinking.
    
    % Paragraph 4: State the main contribution and summarize the experimental results.
    %%CF.5.16: This is a good place to state the main contribution of the paper, and I do not think it is the architecture. I think the main contribution is closer to what you wrote before, except that I would frame it more as a framework for lifelong multi-task/multi-context imitation learning that supports large-scale data collection and thus can produce broad generalization to distinct objects, scenes, and tasks. 
    % Our main contribution tackles the problem of zero-shot generalization by collecting a large, diverse, multi-task imitation learning dataset,
    %%CF.5.29: should have made the problem clear long before this sentence. Also, scaling up generalization sounds weird. We scale/broaden data so that we can generalize. We don't scale the generalization itself.
    % and using it to train end-to-end imitation policies with flexible ways to condition them. To deal with the challenges of evaluating end-to-end generalization systems in the real world, we devise a shared autonomy scheme that simultaneously performs data collection, improves the policy from human corrections, and measures policy performance across a wide family of tasks. 
    \rebuttal{Our main contribution is an empirical study of a large-scale interactive imitation learning system that solves a breadth of tasks, including zero-shot and few-shot generalization to tasks \emph{not seen} during training.}
    %The main contribution of this work is a large-scale interactive imitation learning system that allows policies to solve a breadth of tasks, including tasks \emph{not seen} during training.
    Using this system, we collect a large dataset of 100 robotic manipulation tasks, through a combination of expert teleoperation and a shared autonomy process where the human operator ``coaches'' the learned policy by fixing its mistakes.
    Across \numrobots robots, \numoperators different operators collected \numrobotdemos robot demonstrations that totaled \numdemohours hours of robot time, as well as \numvideos human videos of the same tasks. %Multi-task policies are trained end-to-end on this dataset, mapping pixels directly to controls. 
    At test time,
    %We train multi-task policies end-to-end on this dataset using flexible conditioning modalities such as language or videos of humans, so that at test-time, the robot may be instructed to perform new tasks it was never trained to do.
    %%CF - TODO: the above is a little bit repetitive with third paragraph. Consider reducing repetition without breaking the flow.
    %AI.6.18 - trimming a bit.
    the system is capable of performing \numholdout~unseen manipulation tasks between objects that have never previously appeared together in the same scene.
    %For example, the robot can grasp a banana from a cluttered table and place it into a ceramic bowl, when none of the training data included a banana and ceramic bowl in the same scene.
    These closed-loop visuomotor policies perform asynchronous inference and control at 10Hz, amounting to well over 100 decisions per episode. %Finally, we empirically find that data from human interventions allows for better data that improves overall performance. 
    %%CF: Agreed with Alex's comment that it's a weird thing to end on. I'm not sure where else to put it, so I think the best option would be to comment it out.

    % In particular, 
    %%CF.5.16: The "allowing new capabilities to be added" part is not obvious, especially since nearly all papers that do end-to-end imitation learning to single-task learning.
    %%CF.5.16: It would be a very good idea to be explicit about the problem we are aiming to solve. It is somewhat implicit in the first paragraph, but is never explicitly stated beyond the highest-level of motivation. (A crisp problem statement is important.)
    %%CF.5.16: There is a bit of a disconnect here. The key challenge is that we're aiming to solve relates to generalization, while the next two sentences below focus purely on imitation learning. While, we do make some contributions to imitation learning, I don't think those are the main thing that's new about this paper! I would expect this paragraph to focus more on why prior methods haven't successfully generalized broadly. I think the most relevant works to be discussing would then be works that do have some degree of generalization, e.g. methods that do multi-task imitation learning, few-shot imitation learning, or imitation learning in diverse environments (though I don't know any in the latter category in the realm of manipulation). Then, you can say something along the lines of how zero-shot generalization to new scenes and new tasks remains a major challenge, and why it remains a major challenge, i.e. the need to scale up and all of the challenges associated with scaling up!
    % However, there are two major challenges with end-to-end imitation learning. The first is the challenge of \emph{compounding errors}, where imitation learning policies that drift off the expert state distribution do not know how to return to the expert trajectory distribution. % cite ALVINN paper?
    % A number of recent works have proposed solutions \todo{cite DAgger}. The second Although prior work have suggested simulated evaluation, off-policy metrics, \todo{cite}, ultimately general end-to-end system must be verified that it generalizes to a variety of real world scenarios. A canonical example of this is the generalization demands of self-driving cars: even though they learn only a single task, it must be tested in thousands of different scenarios and road conditions. 
    

    %%CF.5.16: This paragraph should ideally connect directly to the challenges discussed in the previous paragraph, making it clear how it addresses those challenges.
    % Taking inspiration from human-in-the-loop techniques used in Autonomous Vehicles research \todo{cite hgdagger}, we build a large-scale imitation learning pipeline capable of achieving different kinds of generalization on challenging robotic tasks, while using human-in-the-loop interaction to solve the resource tradeoff between data collection and policy evaluation. % cite HG-Dagger https://arxiv.org/pdf/1810.02890.pdf
    %%CF.5.16: This paragraph is rather terse. It's not clear where the inspiration from autonomous vehicles comes into the picture. It's not clear why this idea enables generalization
    %%EJ.5.19. Generalization requires lots of data -> The more generalization you have,
    %% the more resources you need to evaluate it -> the less data you have. I'm trying to 
    %% argue that human-in-the-loop DAgger collection solves this problem, and this is a technique already used by AV research. I was thinking that drawing a self-driving car analogy to fleet learning can make the approach make more sense to the audience.

    %%CF.5.16: I would avoid the word novel. It's a rather empty word, and we should strive to sell the importance of the work without emphasizing the novelty of the architecture.
    %%EJ.5.19 - fully agree! 
    
    
    % See the supplementary video and website for additional details.
    
    % citation for IL drift?
    % https://papers.nips.cc/paper/1988/file/812b4ba287f5ee0bc9d43bbf5bbe87fb-Paper.pdf
        % Machine-learning algorithms are well-suited to tackle problems of generalization, especially where
    % it would be infeasible to hand-design controllers and state machines to suit every situation and task.  


%===============================================================================

==> LfD_CoRL (1)/C-overview.tex <==
\section{Problem Setup and Method Overview}

\begin{figure}[t]
\centering
\vspace{-0.2cm}
\includegraphics[width=\linewidth]{figures/tasks-tableau.png} 
\caption{\small A subset of training tasks (top row), and a subset of held-out tasks (bottom two rows) used for evaluating zero shot task generalization. Top left: Given a pretrained task embedding computed from human videos or text, \methodname acts as an ``action decoder'' for the task embedding. 
%On the right, the policy predicts 10 waypoints, visualized in red lines and white circles to aid offline evaluation. The expert trajectory for demos and interventions is plotted in blue.
}
\vspace{-0.3cm}
\label{fig:embed}
\end{figure}

% Overview: explain what precisely is the problem (define it!), what are the parts of the method, how the parts fit together etc. After reading the overview, no subsequent section/subsection heading should come as a surprise to the reader

An overview of our imitation learning system is shown in Figure~\ref{fig:overview}. Our goal is to train a conditional policy that can interpret RGB images, denoted $s \in \mathcal{S}$, together with a task command $w \in \mathcal{W}$,
%%SL.6.18: I introduced a symbol for task command (it did not appear that there was one in the paper before), please select whatever symbol you want, but we should definitely have one.
which might correspond to a language string or a video of a person.
\rebuttal{Different tasks correspond to completing distinct objectives; some example tasks and corresponding commands are shown in Figure~\ref{fig:embed}.}
The policy is a mapping from images and commands to actions, and can be written as $\mu : \mathcal{S} \times \mathcal{W} \rightarrow \mathcal{A}$, where the action space $\mathcal{A}$ consists of the 6-DoF pose of the end effector as well as a 7$^\text{th}$ degree of freedom for continuous control of the parallel jaw gripper.

The policy is trained using a large-scale dataset collected via a VR-based teleoperation rig (see Figure~\ref{fig:overview}, left) through a combination of direct demonstration
%as well as a human-in-the-loop shared autonomy setup (Section~\ref{method:daggercollect}),
and human-in-the-loop shared autonomy. In the latter,
trained policies are deployed on the robot, and the human operator intervenes to provide corrections when the robot makes a mistake. This procedure resembles the human-gated DAgger (HG-DAgger) algorithm~\cite{kelly2019hgdagger,ross2011reduction}, and provides iterative improvement for the learned policy, as well as a continuous signal that can be used to track the policy's performance. % in terms of the intervention rate. %, which we detail in Section~\ref{method:daggereval}.

The policy architecture is divided into an encoder $q(z|w)$, which processes the command $w$ into an embedding $z \in \mathcal{Z}$,
%(e.g., a language embedding for language, or a learned video embedding for human videos), 
and a control layer $\pi$, which processes $(s, z)$ to produce the action $a$, i.e. $\pi : \mathcal{S} \times \mathcal{Z} \rightarrow \mathcal{A}$. This decomposition is illustrated in Figure~\ref{fig:embed}, with further details in Section~\ref{sec:learning}. It provides our method with the ability to incorporate auxiliary supervision, such as pretrained language embeddings, which help to structure the latent task space and facilitate generalization. In our experiments, we will show that this enables generalization to tasks that were not seen during training, including novel compositions of verbs and objects.

\iffalse
Our goal is to learn a task-conditioned policy $\pi$, which maps a monocular RGB image $I$ and task embeddings $z \in \mathbb{R}^{n}$ to multiple actions to be concurrently executed on a mobile manipulation robot. The mobile manipulator is a 7-DOF robot arm, a 1-DOF gripper (open and close), and a 2 DOF base, giving policy $\pi : I \times z \to \mathbb{R}^7_\text{arm} \times \mathbb{R}_\text{gripper}$. Instead of controlling the arm joints directly, we model actions as the 6-DoF Cartesian pose of the end-effector. This action representation is
%intended to be
flexible enough to handle virtually any task the robot hardware is capable of. 
We denote $\pi$ as $\pi(a|s,z)$, model it as a deep neural network,
%that predicts actions from $I \times z$
and train it using behavior cloning to imitate successful expert demonstrations collected via VR-teleoperation. Task embeddings $z$ are computed from a learned video encoder that embeds videos of humans performing the task, or a pre-trained natural language encoder fed an English text description of the task.
%This is further explained in Section~\ref{method:multitaskcond}.

% Implementing imitation learning at scale requires a custom data management interface for searching and filtering out low-quality demonstrations, and customized featurization schemes for handling 10Hz asynchronous control, which we describe in Section~\ref{sec:reannotation}. 
% EJ.6.16 - potentially remove / move to implementation details?

In Section~\ref{sec:method}, we discuss task setup, a teleoperation interface for data collection that allows the user to provide corrective interventions while the neural network policy is autonomously executing, and human video data col

We show in Sections~\ref{method:daggercollect} and \ref{method:daggereval} that not only does this lead to more efficient use of resources by combining collection and policy evaluation, but is also necessary to combat the ``state drift'' problem of imitation learning. 
\fi

% Extensive policy evaluation is needed to measure learning progress, while extenive data collection is needed to improve generalization, creating a resource trade-off.  as a surrogate metric for measuring performance that does not take away data collection resources for evaluation. On the contrary, we show in that it provides valuable DAgger-style data needed to re-train the policy to learn robust behavior. 

% We use the same neural network architecture to learn three different tasks: , which itself consists of hundreds of training ``sub-tasks''. For bin emptying and door opening, the task embedding $g$ is unused and is set to the zero vector. For multi-task manipulation, $g$ encodes knowledge about what sub-task needs to be done, and can be inferred from natural language or from a video of a human performing the same sub-task. 

==> LfD_CoRL (1)/D-related-work.tex <==
\section{Related Work}
\label{sec:relatedwork}
%%EJ.5.19 - might want to point out that the number of works showing generalization on real robots is far too large to discuss here, but our work is pushing on 1) large 6-dof action space with gripper motion 2) hundreds of closed-loop decisions at 10hz control
%%CF.5.16: I think this sentence on classical method probably isn't needed, since it's addressed in the intro. You could even just skip directly to imitation learning, starting by citing a survey paper on imitation learning and some classic papers like ALVINN
%%CF.5.16: I would avoid saying something negative about RL and instead say that we choose to use imitation learning because of <positive thing about IL>. It's generally better to be positive about what you do than to be negative about what other people do
%%AI.5.27 - reminder that we should make sure we cover a good amount of robotics papers in the cites
%%CF.5.29: this point about sample efficiency is weird because demos and robot samples sort of have different data types, and IL definitely requires more demos than RL. Maybe emphasize the stability of supervised learning instead?
%%AI.6.1: I think it's still important to mention the reduced robot time, can think about a different way to phrase this.

%%CF.5.16: I think it would be worth having a paragraph that discusses prior methods that get broad generalization on real robots with techniques other than imitation learning, e.g:
% Generalization to objects includes: visual foresight papers, supersizing self supervision, qt-opt/mt-opt/etc, some of Andy Zeng's papers, DexNet works and probably other grasping papers
% Generalization to envs probably only includes driving/mobility papers. though, Annie Chen's recent paper on DVD also generalizes to new envs.
% Generalization to new tasks: visual foresight and actionable models, any others? 

%%CF.5.16: Some papers that would be good to cite somewhere:
% all the few-shot imitation learning papers (including Rocky Duan paper, MIL and DAML paper, Stephen James' two papers, the DeepMind paper, and Sudeep Dasari's paper)
% language-conditioned imitation papers, including "grounding language in play", and the NeurIPS 2020 paper from Intel and Arizona
% zero-shot imitation learning paper
% paper from Florida on multi-task imitation


% Abhinav Gupta's  https://arxiv.org/pdf/1807.07049.pdf work on novel object, novel home - but tasks are limited to planar grasping, where we focus on 7-Dof closed-loop  manipulation and mobile manipulation like door opening.



% some recent works with DAgger like ideas
% https://arxiv.org/pdf/2103.11512.pdf - from X 
% https://www.robot-learning.uk/coarse-to-fine-imitation-learning
% intervention weighted regressiona
% paper from deepmind https://arxiv.org/pdf/2103.09016.pdf
% debi's recent video-conditioned imitation


%Robot manipulation has been addressed by several learning methods, such as
Imitation learning has been successful in learning grasping and pick-place tasks from low-dimensional state~\cite{argall2009survey,khansariTRO2011,billard2004discovering,schaal2005learning,chalodhorn2007learning,pastor2009learning,mulling2013learning}. Deep learning has enabled imitation learning directly from raw image observations~\cite{pomerleau1989alvinn,zhang2018deep, rahmatizadeh2018vision}. In this work, we focus on enabling zero-shot \rebuttal{and few-shot} generalization to new tasks in an imitation learning framework.

Multiple prior imitation learning works have achieved different forms of generalization, including one-shot generalization to novel objects~\cite{finn2017one,james2018task,yu2018one,bonardi2020learning,zhou2019watch}, to novel object configurations~\cite{paine2018one}, and to novel goal configurations~\cite{duan2017one,huang2019neural,dasari2020transformers}, as well as zero-shot generalization to new objects~\cite{young2020visual}, scenes~\cite{pathak2018zero}, and goal configurations~\cite{goyal2021zero}. Many of these works adapt to the new scenario by conditioning on a robot demonstration~\cite{finn2017one,james2018task}, a video of a human~\cite{yu2018one,bonardi2020learning}, a language instruction~\cite{stepputtis2020language, lynch2020grounding}, or a goal image~\cite{pathak2018zero}.
%Our system can flexibly condition on either a video of a human or a language instruction.
Our system flexibly conditions on either a video of a human or a language instruction, and we focus on achieving zero-shot \rebuttal{(language) and few-shot (video)} generalization to \emph{entirely new} 7-DoF manipulation tasks on a real robot, including scenarios without goal images and where task-relevant objects are never encountered together in the training data. 

%Few-shot and meta-imitation learning methods~\cite{duan2017one,finn2017one,yu2018one,silver2020few,james2018task,huang2019neural,paine2018one} aim to use a small number of examples of many tasks at train time to learn how to quickly solve a test-time task with a small number of demonstrations (possibly zero). Prior work has conditioned on robot demos~\cite{duan2017one}, used gradient-based meta learning~\cite{finn2017one}, and conditioned on videos from simulation~\cite{james2018task,bonardi2020learning,dasari2020transformers}, and human observation~\cite{yu2018one}. For video-based demos, a common approach is to embed demos into a learned task space~\cite{james2018task,zhou2019watch,bonardi2020learning} used to condition the policy afterwards. Our work is most similar to these context-based methods, with a push towards a wider variety of objects and manipulation skills. However, we also explore utilizing semantic embeddings from other sources like language, rather than exclusively examining end-to-end embedding learning.

%Both methods have different strengths, and for this work we chose to use imitation learning. Our aim is to learn a single model that can achieve many tasks, and since imitation learning does not require defining a reward function, we can avoid needing to implement reward functions for every task we wish to learn. This makes imitation learning a good starting point, given no initial data about the task or environment. In practice, supervised learning objectives tend to be more stable than reinforcement learning, which must optimize through long-term credit assignment \cite{gullapalli1991comparison, henderson2018deep}.

%Scaling data collection is a key aspect of generalization. 
It is standard to collect demonstrations via teleoperation~\cite{calinon2009learning} or kinesthetic teaching~\cite{khansariTRO2011}, and active learning methods such as DAgger~\cite{ross2011reduction} help reduce distribution shift for the learner. Unfortunately, DAgger and some of its variants~\cite{ross2014aggrevate,laskey2017dart} are notoriously difficult to apply to robotic manipulation because they necessitate an interface where the expert must annotate the correct action when not in control of the robot policy. %, for every observed state.
%%CF: removing "for every observed state", because I think that laskey does not require it for every observed state.
Inspired by recent works in autonomous driving, HG-DAgger~\cite{kelly2019hgdagger} and EIL~\cite{spencer2020eil}, our system instead only requires the expert to intervene when they believe the policy is likely to make an error and allows the expert to temporarily take full control to put the policy back on track. The resulting data collection scheme is easy to use and helps address distribution shift. Furthermore, the rate of expert interventions during data collection can be used as a live evaluation metric, which we empirically find correlates with policy success.
%One key development in imitation learning is DAgger~\cite{ross2011reduction}. In DAgger, data collection alternates between the expert demonstrator and the learned policy, which helps reduce distributional shift for the learner. There are several DAgger variants which differ in how they alternate between the learned policy and expert policy~\cite{ross2014aggrevate,laskey2017dart}. Our method is most similar to HGDAgger and EIL~\cite{kelly2019hgdagger,spencer2020eil}, where the expert intervenes only if they believe the policy is likely to make an error, rather than according to a random noise schedule. We chose to do this because random expert interventions can be cumbersome, especially in high frequency manipulation environments. By only intervening in error scenarios, the rate of expert intervention can also be used as a live evaluation metric for the quality of the learned policy.

%%CF: These works are probably the least relevant, so discussion of them should go last.
Beyond imitation learning, generalization has been studied in a number of other robot learning works. This includes works that generalize skills to novel objects~\cite{action_image,pinto2016supersizing,mahler2017dex,kalashnikov2018scalable,hatori2018interactively}, to novel environments~\cite{gupta2018robot}, from simulation to reality~\cite{sadeghi2018sim2real,tobin2018domain,mehta2020active,james2019sim,zhang2019vr}, and to new manipulation skills and objects~\cite{finn2017deep,dasari2019robonet,chebotar2021actionable,kalashnikov2021mt}. We focus on the last case of generalizing to novel tasks, but unlike these prior works, we tackle a large suite of 100 challenging tasks that involve 7 DoF control at 10 Hz and involve more than 100 decisions within an episode to solve the task.



%Prior works have utilized imitation learning~\cite{hussein2017survey,pomerleau1989alvinn,ratliff2007imitation} and reinforcement learning~\cite{akkaya2019solving,gu2017deep} to learn robot manipulation skills that generalize along some axis, such as from simulation to reality~\cite{tobin2018domain,sadeghi2018sim2real,mehta2020active,james2019sim,zhang2019vr}, performing a single grasping or tossing skill on novel objects in the same workspace~\cite{mahler2017dex,mahler2018dex,zeng2020tossingbot,kalashnikov2018scalable,kalashnikov2021mt}, and doing a single skill in diverse environments~\cite{gupta2018robot}. Further works aim towards achieving good multi-task performance, where tasks are described by a 1-hot encoding~\cite{todo}, or by goal images and language~\cite{hatori2018interactively,lynch2020grounding,chebotar2021actionable,pathak2018zero}.

%Our focus is to broaden generalization in all directions: dozens of objects, multiple robots, and several skills (wiping, pushing, picking, placing, knocking over) all together. Due to our focus on broad-domain generalization, we choose to use imitation learning as our learning framework of choice, as collecting expert demonstrations allows us to avoid implementing reward functions for the hundreds of tasks we wish to learn. We aim to demonstrate that given a flexible embedding space over tasks, such as learned encoders over language or human video, imitation learning can generalize from previous tasks to novel ones without requiring any kinesthetic demonstrations in the new task.


%DAgger queries the expert for expert labels randomly every timestep. AggreVaTe additionally requires the expert to take over the demonstration after a randomly picked timestep~\cite{ross2014aggrevate}, and DART injects noise during expert demonstrations~\cite{laskey2017dart}. 
%%CF.5.29: You probably don't need to go into this much detail on how these prior methods work.
%%AI.6.1: commenting out.
%Random expert interventions can be cumbersome, especially in high frequency manipulation environments. Instead we use a protocol similar to HGDAgger and EIL~\cite{kelly2019hgdagger,spencer2020eil}, where the expert intervenes only if they believe the policy is like to make a mistake.

%%CF.5.29: Skipping the rest because it looks like it hasn't been edited since I last looked.
%A common goal in robot learning is to learn a model that generalizes outside its training data. Generalization has been achieved from simulation to reality through domain randomization~\cite{tobin2018domain,sadeghi2018sim2real,mehta2020active,james2019sim,zhang2019vr}, and to objects not seen at train time for grasping and tossing~\cite{mahler2017dex,mahler2018dex,zeng2020tossingbot,kalashnikov2018scalable,kalashnikov2021mt}.
%Recent works have pushed towards generalization across environments~\cite{gupta2018robot},
%as well as models that can perform different tasks depending on how they are conditioned. This is often done with a 1-hot encoding of the task~\cite{}, but recent papers have learned pick behaviors from language or goal image embeddings~\cite{hatori2018interactively,lynch2020grounding,chebotar2021actionable}. Our work aims to create an imitation learning system that is able to condition on and generalize over these flexible input spaces, by conditioning on either unconstrained language descriptions of a task, or third-person video demonstrations of a human performing the task.

==> LfD_CoRL (1)/E-data-collection.tex <==

\section{Data Collection and Workflow}
\label{sec:method}

%AI.6.15 going to try to go full "anvils need to be dropped" mode on why we care about this.
In order for an imitation learning system to generalize to new tasks with zero demonstrations of said task, we must be able to easily collect a diverse dataset, provide corrective feedback, and evaluate many tasks at scale. In this section, we discuss these components of our system.

% In this section we describe our data collection and evaluation setting for a fleet of mobile manipulation robots. The robots are teleoperated via a soft-realtime control loop where base, gripper, and arm motions respond within \todo{50ms} of user input. This fast-mirroring of teleoperated input allows dextrous demonstrations to be provided, with image observations recorded at 10Hz. This allows new robotic capabilities to be added and improved on by simply scaling up the quantity and diversity of demonstrations, and can scale to hundreds or even thousands of tasks without additional task engineering. A human-in-the-loop approach to collecting data also acts as a robust safety layer, allowing us to side-step the issue of safe autonomous data collection by having the human simply intervene when the robot is in an unsafe state. % In Section~\ref{sec:concurenteval} we discuss 

\textbf{System Setup.}
\label{method:tasks-and-system}
Our teleoperation system uses an Oculus VR headset which is attached to the robot's onboard computer via USB cable and tracks two handheld controllers.
The teleoperator stands behind the robot and uses the controllers to operate the robot with a line-of-sight 3rd-person view. The robot responds to the operator's movement in a 10 Hz non-realtime control loop. The relatively fast closed-loop control allows the operator to demonstrate a wide range of tasks with ease and quickly intervene if the robot is about to enter an unsafe state during autonomous execution.
%For example, this interface can be used to perform delicate motor control tasks such as pouring a drink into a cup or grasping a brush and using it to wipe a surface.
%All of our tasks can be demonstrated with the same interface without requiring custom motion primitives.
Further details on the user interface and data collection are in Appendices~\ref{appendix:questcontrol} and~\ref{appendix:datacollect}.

%An Oculus headset is attached to the onboard computer via USB connection, and wirelessly tracks the poses of two handheld controllers. The user teleoperates the robot by standing behind the robot and using the controllers to teleoperate it via line-of-sight, like controlling a 3rd person video game character. The robot responds to user movement in a 10Hz non-realtime control loop, recording images asynchronously at 10Hz. The fast closed-loop control loop of the system allows a wide range of tasks to be demonstrated with with ease and for the human to quickly intervene if the robot is about to enter an unsafe state during autonomous execution. Examples of tasks that can be demonstrated with this interface include grasping a brush and using it to wipe surfaces, pouring a drink into a cup, opening drawers, and pushing down on handles in order to open doors (though in this work we do not attempt to learn these tasks). No custom motion primitives were designed for any of these tasks, and they can all be demonstrated using the same teleoperation interface. Appendix~\ref{appendix:questcontrol} describes additional details of the user interface, and Appendix~\ref{appendix:datacollect} describes additional comments about data collection best practices.

%This flexible interface, in conjunction with imitation learning methods, allow new robotic capabilities to be added and improved on by simply scaling up the quantity and diversity of demonstrations, and we show this by scaling to hundreds of tasks without additional task engineering.

%AI.6.16: revising to describe bin picking and door opening as evaluations in single / few-task settings.

%We collect demonstrations for and evaluate trained imitation learning models on the following tasks:

%\begin{enumerate}
    %\item \textbf{Bin-Picking} The robot grasps 4 objects (a paper cup, paper bowl, plastic bottle, a metal can) from one bin and drops them in an adjacent bin. The robot base relative to the bin and starting configuration of objects are randomly varied between episodes. We train and test on the same environment and set of objects, so the generalization requirements are mild for this task - the policy need only to generalize to object configurations and base offset to the bin.
    %\item \textbf{Pushed Door Opening} The robot opens various conference room doors in office buildings, which can be opened by pushing the handle. The doors swing either left-to-right or right-to-left. The arm configuration is randomized at the beginning of the episode, but otherwise held in a fixed position, and the robot must drive into the door handle at the correct angle, and then enter the conference room without colliding into the door frame or other objects. The robot action commands in this task are forward and steering speeds. We collect a mixture of real and sim data on 21 conference rooms and evaluate on 4 unseen rooms.
    %\item \textbf{Latched Door Opening} The same as swing door opening, except the doors have handles that must be rotated downward before pushing the door open. Compared to the `Pushed Door Opening' task, the task is much harder, since the handle must be turned before the door can be opened. The action command sent to the robot consists of both arm (7-DoF) and base motions (2-DoF). We collect data on 4 conference rooms in sim and real and test on 4 unseen real rooms. 
%\end{enumerate}
\textbf{Environment and Tasks.}
We place each robot in front of a table with anywhere from 6 to 15 household objects with randomized poses. 
%This set-up is designed so that many tasks can be performed from the same initial object configuration, making it easier to collect data for many distinct tasks and forcing the model to infer the task of interest from the command rather than the initial scene. 
We collect demonstrations and videos of humans for 100 pre-specified tasks (listed in Tables~\ref{table:traintasks} and~\ref{table:remainingtrainsubtasks}), 
% Appendix~\ref{appendix:subtask-results}
\rebuttal{which span 9 underlying skills such as pushing and pick-and-place}. The model is then evaluated on 29 \emph{new} tasks using a new language description or video of that task. For the method to perform well on these held-out tasks, it must both correctly interpret the new task command and output actions that are consistent with that task.

%The robot is placed in front of a table with anywhere from 6 to 15 objects with randomized object poses. The robot is provided a description of the desired task, either as a natural language instruction, or a video of a human performing the same task (with their human hands). The setup is designed such that the same object configuration could lead to many different tasks, which forces the model to determine the task of interest from the task description. Demonstrations are collected for 100 pre-specified sub-tasks (Table~\ref{table:traintasks} and Appendix~\ref{appendix:subtask-results}). At evaluation time, we \textit{do not} evaluate on the same sub-tasks. The model is evaluated on 29 new language descriptions and videos. We emphasize that for the model to perform well, it must both correctly interpret the new task description, and output action commands consistent with that new task.

\textbf{Shared Autonomy Data Collection.}
\label{method:daggercollect}
Data collection begins with an initial expert-only phase, where
%a task is randomly sampled and
the human provides the demonstration of the task from start-to-finish.
%Each task begins with an initial ``expert-only collect'' mode, where the human provides the teleoperated demonstration of the commanded task from start to finish. % Using just expert data was sufficient for bin picking and door opening tasks, but did not perform well on the multi-task manipulation task. Solving more tasks require obtaining more examples, and we look towards using DAgger style methods to reduce data needs.
After an initial multi-task policy is learned from expert-only data, we continue collecting demonstrations in ``shared autonomy'' mode, where the current policy attempts
%to execute
the task while the human supervises. At any point the human may take over by gripping an ``override'' switch, which allows them to briefly take full control of the robot and perform necessary corrections when the policy is about to enter an unsafe state, or if they believe the current policy will not successfully complete the task.
%The operator briefly takes full control of the robot to put it back on track. % Letting go of the switch relinquishes control to the autonomous policy. 
%This setup is analogous to the , where the moment of intervention is based on the human's estimate of policy behavior, rather than randomly sampled. Like HG-DAgger, 
This setup enables HG-DAgger~\cite{kelly2019hgdagger}, where intervention data is then aggregated with the existing data and used to re-train the policy. For the multi-task manipulation tasks, we collect \numexpertdemo expert-only demonstrations for the initial policies, then collected an additional \numdaggerdemo HG-DAgger demonstrations
%%CF: Is this number referring to the number of interventions, or the number of episodes with interventions? should clarify.
covering 16 iterations of policy deployment, \rebuttal{where each iteration deploys the most recent policy trained on the aggregated dataset}. This gives a total of \numrobotdemos robot demos. We find in Table~\ref{table:ablation-results} that when controlling for the same number of total episodes, HG-DAgger improves performance substantially. 

\textbf{Shared Autonomy Evaluation.}
\label{method:daggereval}
%As the amount of generalization we expect from an end-to-end model increases (across tasks, object positions, scenes), so does the burden of evaluating many generalization scenarios and tasks in the real world. 
When success rates are low, resources are best spent on collecting more data to improve the policy; but evaluation is also important to debug problems in the workflow. As the expected degree of generalization increases, we need more trials to evaluate the extent of policy generalization. This creates a resource trade-off: how should robot time be allocated between measuring policy success rates and collecting additional demonstrations to improve the policy? 
Fortunately, shared autonomy data collection confers an additional benefit: the \textit{intervention rate}, measured as the average number of interventions required per episode, can be used as an indication for policy performance. In Figure~\ref{fig:success-vs-autonomy}, we find that the intervention rate correlates negatively with overall policy success rate. 
%Not only are human interventions useful for improving policy behavior, but intervention rate serves as a helpful metric for quantifying partial learning progress when the success rate is initially low, such as when a robot tasked with a pick-place behavior can pick the object but fails to place it. 

% \paragraph{Video Data Collection}

%When videos $w \in \mathcal{W}$ are used for task commands, we observe that any video of the task can be used for conditioning. It need not share the same camera viewpoint or arrangement of objects, and it could be performed by a human or a robot. 
%This makes video a very expressive way to describe a task.
%Human videos are more natural to provide for an end user, so w
%These videos have different object configurations from the robot demonstrations, were demonstrated by 7 operators, and in fact are primarily collected in home and office setups different from the building the robot is operated in. In each setup, up to three webcams record a human operator performing the task with their hands, each from different viewpoints. Each viewpoint is treated as a separate video of the task, allowing us to record several video demonstrations at once. We collect \numvideos~human videos in total. This data is substantially easier to collect at scale than the robot demonstrations: on average, we find that the demonstrators complete a task with their hands about 10 times faster than through teleoperation. %record from several cameras at once, and on average operators could complete a task with their hands around 10 times faster than a teleoperated robot.

\iffalse
\todo{remove this if freeform ends up performing worse} Additionally, some video demonstrations were collected for tasks that were not in the 104 prespecified sub-tasks mentioned in Section~\ref{method:tasks-and-system}. The video embedding model had a contrastive loss component in its training setup (see Section~\ref{TODO}). Video demonstrations for completely separate tasks were used as negative examples for the contrastive losses. Although we collected such negative examples ourselves, they could be taken from arbitrary video data sources, such as previously released datasets, or videos scraped from YouTube. We leave this for future work.
\fi

\section{Learning Algorithm}
\label{sec:learning}

The data collection procedure above results in a large multi-task dataset. For each task $i$, this dataset contains expert data $(s,a) \in \mathcal{D}_e^i$, human video data $w_h \in \mathcal{D}_h^i$, and one language command $w_\ell^i$. We now discuss how we use this data to train the encoder $q(z|w)$ and the control layer $\pi(a|s, z)$.
% We now discuss how the video embeddings $q(z|w)$ and policy network $\pi(a|s,z)$ are trained.

\subsection{Language and Video Encoders}

Our encoder $q(z|w)$ takes either a language command $w_\ell^i$ or a video of a human $w_h$ as input and produces a task embedding $z$. If the command is a language command, we use a pretrained multilingual sentence encoder~\citep{yang2019multilingual}\footnote{Checkpoint from \url{https://tfhub.dev/google/universal-sentence-encoder-multilingual/3}} as our encoder, producing a 512-dim language vector for each task. Despite the simplicity, we find that these encoders work well in our experiments.

When task commands are instead a video of a human performing the task, we use a convolutional neural network to produce $z$, specifically a ResNet-18 based model.
%When videos $w \in \mathcal{W}$ are used for task commands, we observe that any video of the task can be used for conditioning. It need not share the same camera viewpoint or arrangement of objects, and could be performed by a human or a robot. 
%This makes video a very expressive way to describe a task.
%Human videos are more natural to provide for an end user, so we collected a dataset of \numvideos videos of humans
%doing various tasks.
%These human videos were demonstrated by 7 operators in a variety of buildings and home environments. To speed up data collection, each episode was recorded from multiple cameras, with each camera viewpoint treated as a separate video.
Inspired by recent works~\cite{yu2018one,james2018task}, we train this network in an end-to-end manner. We collected a dataset of \numvideos videos of humans doing each training task, in a variety of home and office locations, camera viewpoints, and object configurations.
Using paired examples of a human video $w_h^i$ and corresponding demonstration demo $\{(s,a)\}^i$, we encode the human video $z^i\sim q(\cdot \mid w_h^i)$, then pass the embedding to the control layer $\pi(a|s,z^i)$, and then backpropagate gradient of the behavior cloning loss to both the policy and encoder parameters.
%The encoded human video $q(z|w)$ conditions the control layer $\pi(a|s,z)$, which is updated to minimize imitation learning loss, and these gradients backprop through the encoder $q$.
%Additionally, since robot demos double as videos of the task, we encode the robot video with the same encoder $q$, treating this as a positive pair for a contrastive loss.

Visualizations of learned embeddings in Appendix~\ref{appendix:video} indicate that by itself, this end-to-end approach tends to overfit to initial object scenes, learn poor embeddings, and show poor task generalization. To help align the video embeddings more semantically, we therefore further introduce an auxiliary \textit{language regression} loss. Concretely, this auxiliary loss trains the video encoder to predict the embedding of the task's language command with a cosine loss. The resulting video encoder objective is as follows:
\begin{equation}
\min \sum_{\text{task } i} \sum_{\substack{
(s,a) \sim \mathcal{D}_e^i \\ w_h\sim\mathcal{D}_h^i \bigcup \mathcal{D}_e^i}} 
\underbrace{-\log \pi(a | s, z^i)}_{\text{behavior cloning}} + \underbrace{D_\text{cos}(z^i_h, z^i_\ell)}_{\text{language regression}} \text{, where } \underbrace{ z^i_h\sim q(\cdot | w_h)}_{\text{video encoder}}, \underbrace{ z^i_\ell \sim q(\cdot | w_\ell^i)}_{\text{language encoder}}
\end{equation}
where $D_\text{cos}$ denotes the cosine distance.
%Each example corresponds to one of 100 tasks, each with a sentence description. The sentence descriptions are embedded with a pretrained multilingual sentence encoder~\citep{yang2019multilingual}\footnote{\url{https://tfhub.dev/google/universal-sentence-encoder-multilingual/3}}, producing a 512-dim language vector, and
%Video encoder $q(z|w)$ has an added loss term to predict the language vector with a cosine loss. 
Since robot demos double as videos of the task, we also train encoded robot videos to match to the language vector. This language loss is critical to learning a more organized embedding space. Additional architecture and training details are in Appendix~\ref{appendix:video}.

%We initially tried learning video embeddings without any language input, through self-supervised contrastive losses. Visualizations of learned embeddings in Appendix~\cite{TODO} indicated that contrastive losses tended to overfit to initial object scenes, rather than the demonstrated task. We instead leveraged additional language labels to help align video embeddings in a more semantically meaningful space.
%Each human video corresponds to one of 100 tasks. The sentence description for each of the 100 tasks is embedded with a pretrained multilingual sentence encoder~\citep{yang2019multilingual}\footnote{\url{https://tfhub.dev/google/universal-sentence-encoder-multilingual/3}}, producing a 512-dim language vector, and the video encoder is trained to predict the language vector with a cosine loss.

%Since videos of robot demonstrations are also videos of the task, we include the \numrobotdemos robot demos as additional training data. In addition to the language loss, we included an end-to-end policy loss inspired by Task-Embedded Control~\cite{james2018task}. Each batch is made of paired videos $(w_{human}, w_robot)$. 
%for every task, a video $w$ is first encoded via $q(z|w)$. The embedding $z$ then conditions policy $\pi(a|s,z)$, which is updated to minimize imitation learning loss, whose gradients backprop from $\pi$ through $q$. The batch is always balanced to be 50\% human video and 50\% robot videos. We emphasize that although robot videos and actions are given at train time, inference is always based on providing a human demonstration without actions.

%were included as additional data, and since these robot demos also contained expert actions, for robot videos we instantiate an instance of the policy and allow the BC loss to backprop from the policy through the video embedding.

%During training, videos $w$ are randomly subsampled to be 20 frames long, done such that the first and last frame of the video remain in the subsampled $w$. The same image augmentations used for training the policy are applied to the video, but we additionally apply random reflections along the x-axis and y-axis. The 20 frames are then arranged into a 4x5 array of images that are processed by a 2D ResNet-18 network. Arranging the images in this manner allows the 2D convolutions in the ResNet to perform several layers of temporal convolution without needing to tune a new architecture, and we found this trick saved GPU memory and permitted a 25\% increase in batch size.%on \todo{P100 GPUs}.
%After mean-pooling the final visual features, we add a fully-connected layer with 32 units. The final embedding is normalized to have unit L2 norm. Further details are in the Appendix.

%For video conditioning, we initially applied a method similar to Task-Embedded Control~\cite{james2018task}. A contrastive loss (cosine similarity or InfoNCE~\cite{oord2018representation}) was applied to the videos, along with the end-to-end BC loss. Embedding visualizations (included in the Appendix) revealed that the embeddings learned were subpar, due to grouping videos based on the set of visible objects, rather than the task performed.







%We emphasize that for video conditioning, although robot videos and language are given at train time, inference is always based on providing a human demonstration without actions or language label.
%When tested on a novel task, we collect 10 human videos for that task.
%The mean embedding over 10 videos for each task were used as the embedding for all demos of that task when retraining the policy. At inference time, we average the embeddings of 10 human video demos of the novel task.

%\subsection{Multi-Task Conditioning}

\subsection{Policy Training}
\label{section:policy-training}

Given a fixed task embedding, we train $\pi(a|s,z)$ via Huber loss on XYZ and axis-angle predictions, and log loss for the gripper angle. During training, images are randomly cropped, downsampled, and subjected to standard photometric augmentations. Below we describe two additional design choices that we found to be helpful. Additional training details such as learning rates, batch sizes, pseudocode, and further hyperparameters are discussed in Appendix~\ref{appendix:training}. 


%% Policy training info, not architecture
\textbf{Open-Loop Auxiliary Predictions.} The policy predicts the action the robot would take, as well as an open-loop trajectory of the next 10 actions the policy would take if it were operating in an open-loop manner. At inference time, the policy operates closed-loop, only executing the first action based on the current image. The open-loop prediction confers an auxiliary training objective, and provides a way to visually inspect the quality of a closed-loop plan in an offline manner (see Figure~\ref{fig:overview}, right). %In pick-and-place tasks for instance, the trajectory plan can reveal if the model "knows" which objects it should proceed towards after it has picked up the first object.

\textbf{State Differences as Actions.} In standard imitation learning implementations, actions taken at demonstration-time are used directly as target labels to be predicted from states. However, cloning expert actions at 10Hz resulted in the policy learning very small actions, as well as dithering behavior. To address this, we define actions as state differences to target poses $N>1$ steps in the future, using an adaptive algorithm to choose $N$ based on how much the arm and gripper move. We provide ablation studies for this design choice in Section~\ref{results:ablationsingletask} and further details in Appendix~\ref{appendix:featurization}







\subsection{Network Architecture}
\label{sec:networkarchitecture}
\label{method:multitaskcond}
\begin{figure}[t]
  \centering
    \includegraphics[width=\linewidth]{figures/singletask_architecture_base.png} 
    \caption{\small \methodname network architecture. A monocular RGB image from the head-mounted camera is passed through a ResNet18 encoder, then through a two-layer MLP to predict each action modality (delta XYZ, delta axis-angle, and gripper angle). FiLM layers \cite{perez2018film} condition the architecture on a task embedding $z$ computed from language $w_\ell$ or video $w_h$. %The policy is not jointly trained with the embedding, so in principle any embedding space over tasks can be utilized.
    } % We do not condition on embeddings for the door opening and bin emptying tasks. For door opening, we predict the base forward and yaw velocityies and keep the arm fixed.}
  \label{fig:architecture}
 %\vspace{-10pt}
\end{figure}

We model the policy using a deep neural network, shown in Figure~\ref{fig:architecture}. 
The policy network processes the camera image with a ResNet18 ``torso'' \cite{he2016identity}, which branches from the last mean-pool layer into multiple ``action heads''. Each head is a multilayer perceptron with two hidden layers of size 256 each and ReLU activations, and models part of the end-effector action, specifically the delta XYZ, delta axis-angle, and normalized gripper angle. 
The policy is conditioned on a 512-dim task embedding $z$, through FiLM layers~\citep{perez2018film}. Following~\citet{perez2018film}, the task conditioning is linearly projected to channel-wise scales and shifts for each channel of each of the 4 ResNet blocks.




% The inputs to the network are a single 512x640 RGB image from the monocular camera of the robot, along with a context embedding that encodes optional proprioception or task conditioning information. For door opening tasks, proprioception includes the current 2-dim base velocity.

 %The tool pose and base velocity prediction heads are trained to minimize mean-square-error with the expert labels. The gripper angle is trained using log loss.


%TensorFlow code for the model architecture and hyperparameter configurations are included in the supplemental material. \todo{add hparams in appendix}.




% \begin{figure}[t]
%   \centering
%     \includegraphics[width=0.5\linewidth]{figures/latched_ sim-real.png}
%     \caption{An example of adapting a sim image (left) to look real (right) using RetinaGAN \cite{retinagan2021}.}
%   \label{fig:retinagan}
% \end{figure}



% \subsubsection{Language Embeddings}

% %Given how effective the language objective was at helping align video embeddings in a more semantically meaningful way, can we directly use the language embedder itself, rather than learning an embedding space from video? To test this, the policy is conditioned on sentence embeddings of the train time tasks. 
% We also consider directly conditioning on the language embeddings produced by the language encoder \citet{yang2019multilingual}. At inference time, we provide a sentence describing a new task, and the policy must generalize to the embedding of that new sentence.
% %Note that the language space used was not directly learned for the purpose of robot learning, and there is no end-to-end loss between policy actions and language embedding. Instead 
% The policy must learn to act like a decoder, mapping language embeddings and the current state into actions consistent with that language. Section~\ref{sec:results} demonstrates that the policy can learn to decode this embedding space, achieving zero-shot transfer to language embeddings of tasks that use words not seen during training.
%$and can perform tasks using words not seen during training.

%Each demonstration was labeled with an English sentence description of the task. The sentence was provided to a pretrained multilingual sentence encoder~\citep{yang2019multilingual}\footnote{\url{https://tfhub.dev/google/universal-sentence-encoder-multilingual/3}}, and the resulting embedding was given to the policy. Since the sentence encoder was pretrained on a wide variety of sentences, semantically similar tasks were already embedded to vectors close to one another.

% \subsection{Large-scale teleoperated data collection}
% \label{sec:collect}


% States are performed at a 10Hz frequency, meaning actions come from 10Hz control. Control is performed asynchronously, but actions defined as the delta between states correspond to synchronous actions, causing a mismatch in evaluation. Additionally, expert actions were small in magnitude at this frequency, leading 

% Instead,  This allows us to decouple the action representation used at collection time from the action representation being predicted (for instance, predicting joint angle displacements while the teleoperation interface translates human motion to cartesian commands). The action representation used can effect final performance, even if the demos used are identical~\cite{peng2016terrain}, and this design choice let us quickly evaluate which representations led to better performance. We compared joint angles to Cartesian displacement, axis angle vs quaternions for rotation, and absolute pose vs. pose deltas for end-effector pose. 

%AI.6.14 - making a revision to downplay importance a bit in case reader doesn't really understand
%With 10Hz control, individual expert actions are too small in magnitude, resulting in substantial drift off the expert distribution and dithering behavior of the policy due to the difficulty of cloning this noisy distribution. Skipping a fixed $N$ states ahead to compute the state-diff action allows the robot to move more smoothly towards target objects, but introduces a significant bias: when performing pick-and-place tasks, the $N$-step lookahead of ``gripper closing" is executed before the arm has moved sufficiently close enough to reach the object. We introduce an adaptive state-diff scheme % $N(t) = \min{25, i}$.
% , described in Appendix~\ref{appendix:featurization}.

% We also found it absolutely critical to filter data \todo{describe this}



% Teleoperators can look at other teleoperator demonstrations for same episode to spot inconsistencies with how demonstrations are being provided.



==> LfD_CoRL (1)/F-results.tex <==


Our experiments aim to evaluate \methodname in large-scale imitation learning settings. We start with an initial validation of \methodname on single-task visual imitation learning. Then, our experiments will aim to answer the following questions: (1) Can \methodname enable zero-shot \rebuttal{and few-shot} generalization to new tasks from a command in the form of language or a video of a human? (2) Is the performance of \methodname bottlenecked by the task embedding or by the policy? (3) How important are different components of \methodname, including HG-DAgger data collection and adaptive state diffs? We present experiments aimed at these questions in this section.

% We quantify the generalization capabilities of end-to-end imitation learning on various manipulation tasks. For all success rates we report the mean success rate, with the sample standard deviation in parentheses.

\subsection{\methodname on Single-Task Imitation Learning}
\label{sec:dooropening}

\iffalse %%CF: Commenting this out for space for the rebuttal edits. I'm moving it to appendix H
\begin{figure}[t]
  \centering
    \includegraphics[width=\linewidth]{figures/swing_doors.png}
    \caption{\small Bin Emptying and Door Opening tasks are used to validate that \methodname can achieve a high level of task success and generalize to unseen scenes in a single-task imitation learning setting.}
    \label{fig:singletasks}
    \vspace{-10pt}
\end{figure}
\fi

We first aim to verify that \methodname can learn individual vision-based tasks before considering the more challenging multi-task setting. We choose two tasks: a \textit{bin-emptying} task where the robot must grasp objects from a bin and drop them into an adjacent bin, and a \textit{door opening} task where the robot must push open a door while avoiding collisions. Both tasks use the architecture in Figure~\ref{fig:architecture}, except that the door opening task involves predicting the forward and yaw velocity of the base instead of controlling the arm. The bin-emptying dataset has 2,759 demonstrations, while the door opening dataset has 12,000 demonstrations collected across 24 meeting rooms and 36,000 demonstrations across 5 meeting rooms in simulation. Further task and dataset details are in Appendix~\ref{appendix:door-results}.

\input{singletaskresults}

In Table~\ref{table:door-results}, we see that the \methodname model is able to reach a pick-rate of 3.4 picks per minute,
%albeit at a slower speed than a human teleoperator.
over half the speed of a human teleoperator.
Further, we see that \methodname reaches a success rate of $87\%$ on the training door scenes and $94\%$ on held-out door scenes. These results validate that the \methodname model and data collect system can achieve good performance on both training and held-out scenes in the single-task setting. Additional analysis is provided in Appendix~\ref{appendix:sorty-toy-results}.
%We wanted to verify that \methodname could learn single manipulation tasks, before trying a more ambitious multi-task setup. We choose two tasks, a \textit{bin-picking} task where the robot must grasp objects from a bin and drop them in an adjacent bin, and a \textit{door opening} task where the robot must push open a door without colliding into the door frame or other objects. 
%For bin-picking, we train \methodname on 2759 expert demonstrations, showing in Table~\ref{table:door-results} that it is able to achieve a fairly high pick-rate, albeit at a slower speed than a human teleoperator. 
%For door opening, we use the same architecture described in Figure~\ref{fig:architecture} but predict the forward and yaw velocity of the base instead of the arm motions. 
%We trained a model capable of opening both left and right swing doors, and evaluate it on all 24 meeting rooms seen during training and an additional of 4 holdout rooms (2 left and 2 right swing doors). As shown in Table~\ref{table:door-results}, \methodname can generalize to novel door instances. 


% The robot opens various conference room doors in office buildings, which can be opened by pushing the handle. The doors swing either left-to-right or right-to-left. The arm configuration is randomized at the beginning of the episode, but otherwise held in a fixed position. The robot must drive into the door handle at the correct angle to push it open, then enter the conference room without colliding into the door frame or other objects. The robot action commands in this task are forward and steering speeds. We collect a mixture of real and sim data on 21 conference rooms and evaluate on 4 real unseen rooms.


% To verify that the imitation method proposed above is capable of achieving a high degree of degree of task success by only training on expert demonstrations, Table \ref{table:door-results} provides the evaluation results, indicating the trained model is capable of reaching high performance on both trained and hold out scenes. Figure \ref{fig:door-generalization} illustrates a few snapshots from the evaluations. 




% We evaluated the latched door models on all the four rooms seen during the training and an additional of 4 holdout tasks. Note that this task is significantly harder than opening the pushed doors since the policy needs to accurately navigate the robot in front of the door handle and then to properly manipulate the door handle while coordinating the arm-base movement. Our models achieves the high success rate of 83\% on the seen rooms despite using in total of less than 1K sim and real episodes. The generalization to the holdout rooms however is not as good as the pushed door model, most likely due to the limited number of meeting rooms used in the training.






% \subsection{Can Imitation Learning Generalize to General Task Embeddings?}

% % \todo{argue that video encoder and language embeddings embed task specifications into semantically meaningful task spaces. The question is whether a policy can learn to interpret the space. by de-coupling the training of the embedding from the policy decoding of the embedding, we can study whether the policy decoder can independently generalize to well-structured embedding spaces.}

% %AI.6.16 - doing an attempt at this.

% Theoretically, given a large enough dataset of language instructions paired to robot demonstrations, it would be possible to learn a language task embedding in an end-to-end manner. However, doing so from scratch would require an especially large amount of robot data. In contrast, the field of NLP has released several language understanding models with semantically meaningful embedding spaces~\cite{word2vec,glove,andothers} that have been used for many downstream NLP tasks.

% This leads to a natural question: \textit{can robotic imitation learning be treated as a downstream task to representation learning}? %Viewing the language model as a task encoder $p(z|g)$, a policy can be viewed as a conditional decoder $\pi(a|x, z)$.  Conditioned on an image from the robot camera, the policy must learn to interpret the vector from language embedding space, and output the desired robot action. 

% \todo{we consider two different learned embedding spaces - embeddings over language and embeddings over video.}

% %AI.6.16 - think this isn't quite it...we want to talk about embedding spaces without mentioning what kind of embedding space and then just talk about language / video towards the end?

%%CF: I'm changing this section header because not all of the task embeddings are pre-trained
\subsection{Evaluating Zero-Shot \rebuttal{and Few-Shot} Task Generalization}
\label{sec:metatidy104}


\begin{figure}[t]
  \centering
    \includegraphics[width=\linewidth]{figures/holdout_sequence.png}
    \caption{\small Qualitative examples of \methodname successfully performing held-out tasks.}
    \label{fig:holdoutqualitative}
    \vspace{-10pt}
\end{figure}


Next, we aim to test whether \methodname can achieve generalization to new tasks. Demonstrations are collected across 100 different manipulation tasks, comprising two disjoint sets of objects. Using disjoint sets of objects allows us to specifically test generalization to combinations of object-object pairs and object-action pairs that are not seen together during training.
For the first set of objects, demonstrations are collected across 21 different tasks, listed in Table~\ref{table:traintasks}, which cover a wide range of skills, from pick-and-place tasks to skills that require positioning the object in a certain way, like ``stand the bottle upright''. For the second set of objects, demonstrations are collected for 79 different tasks, including pick-and-place, surface wiping, and object stacking. The latter family has a smaller variety of manipulation behaviors, but is defined over a larger object set with more clutter. Object sets are shown in Appendix~\ref{appendix:datacollect} and a full list of train task sentences are in Appendix~\ref{appendix:subtask-results}.

% A representative set of 8 tasks within the set of 21 tasks was picked to speed up model comparison to baselines; however, final reported results are over all tasks.

We evaluate \methodname on 29 held-out tasks. \rebuttal{Language conditioned policies are given a novel sentence, while video conditioned policies are given the average embedding of a few human videos of the new task.} Four held-out tasks use objects in the 79-task family, whereas 25 tasks are generated by mixing objects between the 21-task family and 79-task family. Thus, the first 4 held-out tasks do not require cross-object set generalization, so they are easier to generalize to. Even so, we find that each of these 4 tasks are sufficiently challenging that training single-task policies on 300+ held-out demos with DAgger interventions completely fails, achieving 0\% task success. This provides a degree of calibration on the difficulty of these tasks. We hypothesize that a major contributing factor to this challenge is the wide range of locations, objects, and distractors that the skills must generalize to in our settings, as well as the wide range of these factors in the training data.

% \input{holdout4ablation}

% For language based models, the model is given the embedding of a new sentence describing the held-out task. For human video models, the model is given the embedding of a new human video for the task.

In Table~\ref{table:holdouttasks}, we see that language-conditioned \methodname is able to generalize zero-shot to both kinds of held-out tasks, averaging at 32\% success and showing non-zero success on \numholdout held-out tasks. Among the \numholdout hold-out tasks with non-zero success rates, \methodname achieves an average success of \holdoutsuccess when conditioned on language embeddings it has never seen. When conditioning on videos of humans, we find that generalization is much more difficult, but that \methodname is still able to generalize to nine novel tasks with a non-zero success rate, particularly when the task does not involve novel object combinations. 
%To the best of our knowledge, these results represent the first example of zero-shot task generalization of complex vision-based manipulations tasks on a real robot.%We also observe that the language conditioned policy is able to leverage semantically similar embeddings from the language model: commanding ``place food in tray'' and ``place pepper in tray'' generate the same behavior, even though the policy has never been trained on embeddings of the token ``food''.%\methodname generally struggles with wiping tasks and circular motion tasks.%where the robot must perform counterclockwise or clockwise movements. We hypothesize that it is due to the multi-modal nature of the expert trajectories;%These tasks have back-and-forth motions and we hypothesize that the lack of memory in the network makes learning difficult. %lacking memory, the network is unable to commit to a single direction.
Qualitatively, we observe that the language-conditioned policy usually moves towards the correct objects, clearly indicating that the task embedding is reflective of the correct task, as we further illustrate in the supplementary video. The most common source of failures are ``last-centimeter'' errors: failing to close the gripper, failing to let go of objects, or a near miss of the target object when letting go of an object in the gripper.

\input{holdout_task_results_withskill}

\textbf{Is Performance Bottlenecked on the Encoder or the Policy?} Now that we see that \methodname can generalize to a substantial number of held-out tasks to some degree, we ask whether the performance is
\begin{wraptable}{r}{5.5cm}
\small
%\vspace{-0.4cm} % -0.6
\caption{\small Training vs. generalization performance, averaged across 21 of the training tasks and all 28 held-out tasks.}
\vspace{-0.4cm}
\label{tbl:traintest}
\begin{tabular}{llc}\\\toprule  
\textbf{Setting} & \!\!\!\textbf{Task Conditioning}\!\!\! & \textbf{Success} \\
\midrule
\multirow{3}{*}{Train} & One-hot & 42\%\\  
& Language & 40\%\\  
& Video & 24\%\\  
\midrule
\multirow{2}{*}{Held-Out}& Language & 32\% \\
& Video & 4\% \\
\bottomrule
\end{tabular}\vspace{-0.4cm}
\end{wraptable}   limited more by the generalization of the encoder $q(z|w)$, the control layer $\pi(a|s,z)$, or both. To disentangle these factors, we measure the policy success rate on the training tasks conditioned in 
three ways:  a one-hot task identifier, language embeddings of the training task commands, and video embeddings of \textit{held-out} human videos of the training tasks. This comparison is in Table~\ref{tbl:traintest}.
The similar performance between one-hot and language suggests the latent language space is sufficient, and that language-conditioned performance on held-out tasks is bottlenecked on the control layer more than the embedding.
The more significant drop in performance of video-conditioned policies suggests inferring tasks from videos is much more difficult, particularly for held-out tasks.
%Video embeddings perform less well, likely because policy is evaluated using held-out videos of the task, which adds generalization difficulty.
% One way to verify that the policy is able to interpret task embeddings correctly is to verify that it is capable of memorizing a discrete set of task embeddings. We compare language-conditioned and video-conditioned \methodname to a one-hot encoding of training tasks in the 21-task family, showing in Table~\ref{table:traintasks} that \todo{reach comparable success rates} 


% 104-task family models
% \begin{table}
%   \caption{Multi-Task Manipulation Results on different conditioning modalities, aggregated across all trials}
%   \label{table:m104-results}
% \begin{center}
% \begin{tabular}{llll}
% \toprule
% Method & 8 Task & 21-Task & Held-Out Tasks \\
% \midrule
% % Ablations of different conditioning modalities.
% 21-Task w/ One-Hot Vector  & 50\% (4.2) & 54\% (3.5) & N/A \\ % potentially b/190944624
% 21-Task Only w/ Language Embedding & 43\% (2.6) & \todo{40\%} (2.1) & N/A \\ % 
% 100-Task w/ Language Embedding &  &  &  \\ % b/190960290
% 100-Task w/ Human Video Embedding & & \todo{todo\%} & \todo{19\%} (so far) \\
% % Our best models with all data available 
% % Training on holdout tasks & & \todo{70\%}\% & \todo{50\%} \\
% \bottomrule
% \end{tabular}
% \end{center}
% \end{table}

\subsection{Ablation Studies and Comparisons}
\label{results:ablationsingletask}

We validate the importance of several \methodname design decisions using the (training) 21-task family. 
% First, we compare one-hot conditioning to language conditioning on models trained only using the 21-task demonstrations. Performance between the two are fairly similar. \todo{decide on what commentary. They're each over 1 stddev from each other}. 
Our first set of ablations evaluate on the ``place the bottle in ceramic bowl'' command, which has the most demos (1000) of any task. We first test whether multi-task training is helpful for performance: we compare the multi-task system trained on \numrobotdemos demos across all tasks, to a single-task policy trained on just the 1000 demos for the target task. 
In Table~\ref{table:ablation-results} (left), the single-task baseline achieves just 5\% success. The low number is consistent with the low single-task performance on holdout tasks from Section~\ref{sec:metatidy104}: collecting data over several robots and operators likely makes the task harder to learn. Only when pooling data across many tasks does \methodname learn to solve the task. We ablate the adaptive state diff scheme described in Section~\ref{sec:networkarchitecture} and find that it is important; when naively choosing the $N=1$ future state to compute the expert actions, the policy fits the noise and moves too slowly, resulting in state drift away from good trajectories. %This achieves only 3\% success.

\iffalse
\begin{table}
\vspace{-15pt}
\small
  \caption{\small Ablation Studies. All evaluations done on the `place the bottle in the ceramic bowl' task.}
  \label{table:ablation-results}
\begin{center}
\begin{tabular}{llll}
\toprule
\textbf{Method} & \textbf{1-Task Performance} \\
\midrule
% Top-level performance to compare against.
Multi-task system, language conditioned & 52\% (6.3) \\
% Baseline
Multi-task system, one-hot conditioned & 45\% (5.3) \\ % get number from samurai pickplace of the system
Single-task baseline (1000 demos) & 5\% (2.8) \\ % TODO
% Multi-task, No Data Filtering & \todo{TODO} \\ % TODO
Multi-task, one-hot, no adaptive state-diff & 3\% (2.3) \\ % b/189938111
%\midrule
\bottomrule
\end{tabular}
\end{center}
\end{table}
\begin{table}
\vspace{-15pt}
\small
  \caption{\small DAgger comparison on 'place the bottle in the ceramic bowl' (1-Task) and the 8-Task subset from Table~\ref{table:traintasks}. Controlled for the same amount of data, DAgger reaches higher success numbers significantly more quickly.}
  \label{table:dagger}
\begin{center}
\begin{tabular}{lll}
\toprule
\textbf{Dataset} & \textbf{1-Task} & \textbf{8-Task}  \\
\midrule
% Baseline
% Impact of DAgger
100\% Manual & 27\% (5.2)  & 23\% (4.2)\\
50\% Manual +  50\% HG-DAgger  & 53\% (5.8) &  47\% (5.2)\\
\bottomrule
\end{tabular}
\end{center}
  \vspace{-20pt}
\end{table}
\fi

\input{Z-ablation-tables}

\begin{wrapfigure}{r}{0.44\textwidth}
\vspace{-20pt}
  \begin{center}
    %\includegraphics[width=0.48\textwidth]{figures/mean_interventions_success_rate.png}
    \includegraphics[width=0.4\textwidth]{figures/interventions_vs_success.png}
  \end{center}
  \vspace{-0.4cm}
  \caption{\small Mean number of interventions vs. task success rate. Each point represents a policy evaluated during HG-DAgger data collection. There is a clear correlation between the mean number of interventions and success rate, suggesting that interventions can be used as a live proxy for performance.}
  %approaching 100\% as mean interventions reaches 0.}
  \label{fig:success-vs-autonomy}
  \vspace{-20pt}
\end{wrapfigure}
We next ablate the use of HG-DAgger while keeping the total amount of data fixed. Specifically, we compare performance of policies trained using 50\% expert demos and 50\% HG-DAgger interventions, versus using 100\% expert demos. In Table~\ref{table:ablation-results} (right), we find that HG-DAgger significantly improves task performance over cloning expert demonstrations on both the `place bottle in ceramic bowl' task and 7 other training tasks. Further details on this comparison are in Appendix~\ref{app:ablationdetails}.
%% Need to list out the other training tasks.
Finally, in Figure~\ref{fig:success-vs-autonomy}, we evaluate whether measuring HG-DAgger interventions can give us a live proxy of policy performance. We see that intervention frequency is inversely correlated with policy success, as measured by the fraction of successful episodes not requiring intervention. This result suggests that we can indeed use this metric with HG-DAgger for development purposes.

==> LfD_CoRL (1)/Z-ablation-tables.tex <==



\begin{table}[t]
\vspace{-15pt}
\small
  \caption{\small Ablation Studies. Left: Multi-task vs. single task models on the `place the bottle in the ceramic bowl' task. Training across tasks and with adaptive state-diffs is important for good training performance. Right: DAgger comparison on 'place the bottle in the ceramic bowl' (1-Task) and the 8-Task subset from Table~\ref{table:traintasks}. Controlled for the same amount of data, DAgger reaches higher success numbers significantly more quickly.}
  \label{table:ablation-results}
    %\label{table:dagger}
\begin{center}
\begin{tabular}{llll}
\toprule
\textbf{Method} & \textbf{1-Task} \\
\midrule
% Top-level performance to compare against.
Multi-task, language conditioned & 52\% (6.3) \\
% Baseline
Multi-task, one-hot conditioned & 45\% (5.3) \\ % get number from samurai pickplace of the system
Single-task baseline (1000 demos) & 5\% (2.8) \\ % TODO
% Multi-task, No Data Filtering & \todo{TODO} \\ % TODO
Multi-task, one-hot, no adaptive state-diff & 3\% (2.3) \\ % b/189938111
%\midrule
\bottomrule
\end{tabular}
\hfill
\begin{tabular}{p{2.5cm} p{1.3cm} p{1.3cm}}
\toprule
\textbf{Dataset} & \textbf{1-Task} & \textbf{8-Task}  \\
\midrule
% Baseline
% Impact of DAgger
100\% Manual & 27\% (5.2)  & 23\% (4.2)\\
50\% Manual +\newline 50\% HG-DAgger  & 53\% (5.8) &  47\% (5.2)\\
\bottomrule
\end{tabular}
\end{center}
  \vspace{-20pt}
\end{table}


==> LfD_CoRL (1)/abridged_21task_results.tex <==

\begin{table}
\small
  \caption{\small Performance comparsion one-hot, language, or video conditioning over 21 training tasks. Video policies are conditioned on held-out videos of the training tasks.}
  \label{table:traintasks}
\begin{center}
% \begin{tabular}{p{6.5cm} p{1.5cm} p{2cm} p{2cm} p{2cm}}
% \resizebox{\columnwidth}{!}{
\begin{tabular}{lp{2cm}lll}
\toprule
\textbf{Embedding} & \textbf{21 train tasks} \\
\midrule
One-Hot & 42\%\\
Language &  40\% \\
Video & 24\%\\
\bottomrule
\end{tabular}
% }
\end{center}
\end{table}


==> LfD_CoRL (1)/holdout4ablation.tex <==

\begin{wraptable}{r}{9cm}
\vspace{-15pt}
\small
  \caption{\small The holdout tasks are difficult, even when training directly on 300+ demos.}
  \label{table:single-holdout-ablation}
\begin{center}
\begin{tabular}{ll}
\toprule
\textbf{Baseline} & \textbf{Success \%} \\
\midrule
`place apple in paper cup' (63 expert, 355 DAgger) & 0\% (0) \\
`wipe tray with sponge' (65 expert, 262 DAgger) & 0\% (0) \\
`place grapes in red bowl'  (60 expert, 317 demos) & 0\% (0) \\
`place sponge in tray' (85 expert, 300 demos) & 0\% (0) \\ 
%\midrule
\bottomrule
\end{tabular}
\end{center}
\vspace{-15pt}
\end{wraptable}

==> LfD_CoRL (1)/holdout_task_results.tex <==
\begin{table}[t]
\small
  \caption{\small Evaluating zero-shot task generalization. The first 4 tasks only use objects from the 79-task family. The remaining tasks mix objects between the 21-task and 79-task families, requiring further generalization. Numbers in parentheses are 1 unit standard deviation. The language conditioning generalizes to several holdout tasks, whereas the video conditioning shows promise on tasks that do not mix objects between task families.
  %Demo length is not provided because we did not collect start-to-finish expert demos for these tasks.
  %EJ.6.18 - commented out because i think a reviewer who wonders it and cares enough should be able to figure it out. Also, we *could* get these numbers.
  }
  \label{table:holdouttasks}
\begin{center}
\begin{tabular}{p{5.3cm} p{3.2cm} p{3.2cm}}
\toprule
\textbf{Holdout tasks \newline (no demos during training)} & \textbf{Lang-conditioned\newline performance} & \textbf{Video-conditioned\newline performance} \\
\midrule
`place sponge in tray' & 82\% (9.2) & 22\% (2.2) \\
`place grapes in red bowl' & 75\% (10.8) & 12\% (7.8) \\
`place apple in paper cup' & 33\% (12.2) & 14\% (7.8) \\
`wipe tray with sponge' & 0\% (0) & 28\% (10.6) \\
\midrule
`place banana in ceramic bowl' & 75\% (9.7) & 7.5\% (4.2) \\
`place bottle in red bowl' & 75\% (9.7) & 0\% (0) \\
`place grapes in ceramic bowl' & 70\% (10.3) & 0\% (0) \\
`place bottle in table surface' & 50\% (11.2) & 5\% (3.5) \\
`place white sponge in purple bowl' & 45\% (11.2) & 0\% (0) \\
`place white sponge in tray' & 40\% (11.0) & 0\% (0) \\
`place apple in ceramic bowl' & 20\% (8.9) & 0\% (0) \\
`place bottle in purple bowl' & 20\% (8.9) & 0\% (0) \\
%`place plastic cup in the ceramic bowl' & 0\% (0) & N/A \\
`place banana in ceramic cup' & 0\% (0) & 0\% (0) \\
`place banana on white sponge' & 0\% (0) & 0\% (0) \\
`place metal cup in red bowl' & 0\% (0) & 0\% (0) \\
`pick up grapes' & 65\% (10.7) & 0\% (0) \\
`pick up apple' & 55\% (11.2) & 5\% (3.5) \\
`pick up towel' & 42.8\% (18.7) & 0\% (0) \\
`pick up pepper' & 35\% (10.7) & 12.5\% (5.2) \\
`pick up bottle' & 30\% (10.3)& 17.5\% (6.0) \\
`pick up the red bowl' & 0\% (0) & 0\% (0) \\
`drag grapes across the table' & 14\% (13.2) & 0\% (0) \\
`wipe table surface with banana' & 10\% (6.7) & 0\% (0) \\
`wipe tray with white sponge' & 0\% (0) & 0\% (0) \\
`wipe ceramic bowl with brush' & 0\% (0) & 0\% (0) \\
`push purple bowl across the table' & 30\% (10.3) & 0\% (0) \\
`push tray across the table' & 25\% (9.7) & 0\% (0) \\
`push red bowl across the table' & 0\% (0) & 0\% (0) \\
\midrule
\textit{Holdout Task Overall} & 32\% & 4\% \\
\bottomrule
\end{tabular}
\end{center}
\end{table}


==> LfD_CoRL (1)/holdout_task_results_withskill.tex <==
\begin{table}[t]
\scriptsize
  \caption{ Success rates for zero-shot \rebuttal{(language) and few-shot (video)} generalization to tasks not in the training dataset. The first 4 tasks only use objects from the 79-task family. The remaining tasks mix objects between the 21-task and 79-task families, requiring further generalization. Numbers in parentheses are 1 unit standard deviation. The language conditioning generalizes to several holdout tasks, whereas the video conditioning shows promise on tasks that do not mix objects between task families. Overall performance improves slightly with fewer distractor objects.
  }
  \label{table:holdouttasks}
\begin{center}
\begin{tabular}{p{1.2cm} p{4cm} p{2.2cm} p{2.2cm} p{2.2cm}}
\toprule
\textbf{Skill} &\textbf{Held-out tasks \newline (no demos during training)} &
\textbf{Lang-conditioned\newline (1 distractor)} & \textbf{Lang-conditioned\newline (4-5 distractors)} & \textbf{Video-conditioned\newline (4-5 distractors)} \\
\midrule
\multirow{3}{*}{pick-place} &`place sponge in tray' & 83\% (6.8) & 82\% (9.2) & 22\% (2.2) \\
&`place grapes in red bowl' & 87\% (6.2) & 75\% (10.8) & 12\% (7.8) \\
&`place apple in paper cup' & 30\% (8.4) & 33\% (12.2) & 14\% (7.8) \\
\arrayrulecolor{black!30}\cmidrule{2-5}
\multirow{1}{*}{pick-wipe} &`wipe tray with sponge' & 40\% (8.9) & 0\% (0) & 28\% (10.6) \\
\arrayrulecolor{black}\midrule
\multirow{11}{*}{pick-place} &`place banana in ceramic bowl' & 50\% (15.8) & 75\% (9.7) & 7.5\% (4.2) \\
&`place bottle in red bowl' & 50\% (15.8)& 75\% (9.7) & 0\% (0) \\
&`place grapes in ceramic bowl' & 70\% (14.5) & 70\% (10.3) & 0\% (0) \\
&`place bottle in table surface' & 0 & 50\% (11.2) & 5\% (3.5) \\
&`place white sponge in purple bowl' & 70\% (14.9)& 45\% (11.2) & 0\% (0) \\
&`place white sponge in tray' & 50\% (15.8) & 40\% (11.0) & 0\% (0) \\
&`place apple in ceramic bowl' & 30\% (14.5) & 20\% (8.9) & 0\% (0) \\
&`place bottle in purple bowl' & 30\% (14.5) & 20\% (8.9) & 0\% (0) \\
%`place plastic cup in the ceramic bowl' & 0\% (0) & N/A \\
&`place banana in ceramic cup' & 10\% (9.5) & 0\% (0) & 0\% (0) \\
&`place banana on white sponge' & 40\% (15.5) & 0\% (0) & 0\% (0) \\
&`place metal cup in red bowl' & 0\% (0) & 0\% (0) & 0\% (0) \\
\arrayrulecolor{black!30}\cmidrule{2-5}
\multirow{6}{*}{grasp} &`pick up grapes' & 70\% (14.5) & 65\% (10.7) & 0\% (0) \\
&`pick up apple' & 20\% (12.7) & 55\% (11.2) & 5\% (3.5) \\
&`pick up towel' & 50\% (15.8) & 42.8\% (18.7) & 0\% (0) \\
&`pick up pepper' & 50\% (15.8)  & 35\% (10.7) & 12.5\% (5.2) \\
&`pick up bottle' & 40\% (15.5) & 30\% (10.3)& 17.5\% (6.0) \\
&`pick up the red bowl' & 30\% (14.5) & 0\% (0) & 0\% (0) \\
\arrayrulecolor{black!30}\cmidrule{2-5}
\multirow{1}{*}{pick-drag} &`drag grapes across the table' & 0\% (0) & 14\% (13.2) & 0\% (0) \\
\arrayrulecolor{black!30}\cmidrule{2-5}
\multirow{3}{*}{pick-wipe} &`wipe table surface with banana' & 0\% (0) & 10\% (6.7) & 0\% (0) \\
&`wipe tray with white sponge' & 20\% (12.7) & 0\% (0) & 0\% (0) \\
&`wipe ceramic bowl with brush' & 10\% (9.49) & 0\% (0) & 0\% (0) \\
\arrayrulecolor{black!30}\cmidrule{2-5}
\multirow{3}{*}{push} &`push purple bowl across the table' & 50\% (15.8) & 30\% (10.3) & 0\% (0) \\
&`push tray across the table' & 30\% (14.5) & 25\% (9.7) & 0\% (0) \\
&`push red bowl across the table' & 60\% (15.5) & 0\% (0) & 0\% (0) \\
\arrayrulecolor{black}\midrule
&\textit{Holdout Task Overall} & 38\% & 32\% & 4\% \\
\bottomrule
\end{tabular}
\end{center}
\vspace{-15pt}
\end{table}


==> LfD_CoRL (1)/preamble.tex <==
% Use  this to define usepackage macros and shortcuts
\usepackage{graphicx}
\usepackage{booktabs}
% subfigures and subcaptions
\usepackage{caption}
\usepackage{subcaption}
% \newcommand{\todo}[1]{\textcolor{red}{#1}}
\usepackage{longtable}
\usepackage{multirow}
\usepackage[table]{xcolor}



\usepackage{amsfonts} % mathbb
\usepackage{amsmath} % text
\usepackage{amssymb} % other misc math symbols

\usepackage{xspace}
\PassOptionsToPackage{sort}{natbib}


% Important statistics
\newcommand{\numholdout}{24\xspace} % note, this is for non-zero success tasks on language
\newcommand{\holdoutsuccess}{44\%\xspace} % note, this is for non-zero success tasks on language
\newcommand{\numexpertdemo}{11,108\xspace}
\newcommand{\numdaggerdemo}{14,769\xspace}
\newcommand{\numrobotdemos}{25,877\xspace}
\newcommand{\numrobots}{12\xspace}
\newcommand{\numoperators}{7\xspace}
\newcommand{\numdemohours}{125\xspace}
\newcommand{\numvideos}{18,726\xspace}


\newcommand{\holdoutAsuccess}{47\%\xspace}
\newcommand{\holdoutBsuccess}{29\%\xspace}


\newcommand{\eighttask}{\textsuperscript{8}\xspace}
\newcommand{\methodname}{BC-Z\xspace}
% exponent numbers e.g. \expnumber{5}{-3}
\newcommand{\expnumber}[2]{{#1}\mathrm{e}{#2}}
\newcommand{\D}{\mathcal{D}}
\newcommand{\loss}{\mathcal{L}}
\usepackage{wrapfig}
\usepackage{todonotes}
\newcommand*{\rebuttal}{\textcolor{black}}
\usepackage{hyperref}


% \usepackage[noend]{algorithmic}
\usepackage[ruled,vlined]{algorithm2e}
\SetKwInput{KwInput}{Input}

% for handling author affiliations
% \usepackage{authblk}


%\usepackage{titlesec}
%\titlespacing\section{0pt}{0pt plus 2pt minus 2pt}{0pt plus 2pt minus 2pt}
%\titlespacing\subsection{0pt}{3pt plus 4pt minus 2pt}{0pt plus 2pt minus 2pt}
%\titlespacing\subsubsection{0pt}{3pt plus 4pt minus 2pt}{0pt plus 2pt minus 2pt}


==> LfD_CoRL (1)/singletaskresults.tex <==
\begin{wraptable}{r}{7cm}
  \vspace{-12pt}
\small
 \caption{\small Single-task bin and door performance, average and standard deviation across runs.}
 \vspace{-0.1cm}
 \begin{tabular}{lll}
 \toprule
\textbf{Bin-Emptying} & \textbf{Picks / Minute} & \textbf{\# Runs}\\
\midrule
% Baseline
% Our best models with all data available 
Human Expert & 6.3 (2.1) & 2759 \\
\methodname (2759 demos) & 3.4 (1.2) & 9 \\
\midrule
\textbf{Door Opening} & \textbf{Success Rate} & \textbf{\# Runs}\\
\midrule
% Baseline
% Our best models with all data available 
\methodname (24 Train Doors) & 87\% (2.2) & 480 \\
\methodname (4 Holdout Doors) & 94\% (2.7) & 80 \\% b/189150818

%\hline
% 4 Latched Training Doors & 83\% (6) & 40\\ % 
% 4 Latched Holdout Doors & 27\% (7.1) & 40% 
\bottomrule
\end{tabular}
  \label{table:door-results}
  
  \vspace{-15pt}
\end{wraptable} 



==> abridged_21task_results.tex <==

\begin{table}
\small
  \caption{\small Performance comparsion one-hot, language, or video conditioning over 21 training tasks. Video policies are conditioned on held-out videos of the training tasks.}
  \label{table:traintasks}
\begin{center}
% \begin{tabular}{p{6.5cm} p{1.5cm} p{2cm} p{2cm} p{2cm}}
% \resizebox{\columnwidth}{!}{
\begin{tabular}{lp{2cm}lll}
\toprule
\textbf{Embedding} & \textbf{21 train tasks} \\
\midrule
One-Hot & 42\%\\
Language &  40\% \\
Video & 24\%\\
\bottomrule
\end{tabular}
% }
\end{center}
\end{table}


==> holdout4ablation.tex <==

\begin{wraptable}{r}{9cm}
\vspace{-15pt}
\small
  \caption{\small The holdout tasks are difficult, even when training directly on 300+ demos.}
  \label{table:single-holdout-ablation}
\begin{center}
\begin{tabular}{ll}
\toprule
\textbf{Baseline} & \textbf{Success \%} \\
\midrule
`place apple in paper cup' (63 expert, 355 DAgger) & 0\% (0) \\
`wipe tray with sponge' (65 expert, 262 DAgger) & 0\% (0) \\
`place grapes in red bowl'  (60 expert, 317 demos) & 0\% (0) \\
`place sponge in tray' (85 expert, 300 demos) & 0\% (0) \\ 
%\midrule
\bottomrule
\end{tabular}
\end{center}
\vspace{-15pt}
\end{wraptable}

==> holdout_task_results.tex <==
\begin{table}[t]
\small
  \caption{\small Evaluating zero-shot task generalization. The first 4 tasks only use objects from the 79-task family. The remaining tasks mix objects between the 21-task and 79-task families, requiring further generalization. Numbers in parentheses are 1 unit standard deviation. The language conditioning generalizes to several holdout tasks, whereas the video conditioning shows promise on tasks that do not mix objects between task families.
  %Demo length is not provided because we did not collect start-to-finish expert demos for these tasks.
  %EJ.6.18 - commented out because i think a reviewer who wonders it and cares enough should be able to figure it out. Also, we *could* get these numbers.
  }
  \label{table:holdouttasks}
\begin{center}
\begin{tabular}{p{5.3cm} p{3.2cm} p{3.2cm}}
\toprule
\textbf{Holdout tasks \newline (no demos during training)} & \textbf{Lang-conditioned\newline performance} & \textbf{Video-conditioned\newline performance} \\
\midrule
`place sponge in tray' & 82\% (9.2) & 22\% (2.2) \\
`place grapes in red bowl' & 75\% (10.8) & 12\% (7.8) \\
`place apple in paper cup' & 33\% (12.2) & 14\% (7.8) \\
`wipe tray with sponge' & 0\% (0) & 28\% (10.6) \\
\midrule
`place banana in ceramic bowl' & 75\% (9.7) & 7.5\% (4.2) \\
`place bottle in red bowl' & 75\% (9.7) & 0\% (0) \\
`place grapes in ceramic bowl' & 70\% (10.3) & 0\% (0) \\
`place bottle in table surface' & 50\% (11.2) & 5\% (3.5) \\
`place white sponge in purple bowl' & 45\% (11.2) & 0\% (0) \\
`place white sponge in tray' & 40\% (11.0) & 0\% (0) \\
`place apple in ceramic bowl' & 20\% (8.9) & 0\% (0) \\
`place bottle in purple bowl' & 20\% (8.9) & 0\% (0) \\
%`place plastic cup in the ceramic bowl' & 0\% (0) & N/A \\
`place banana in ceramic cup' & 0\% (0) & 0\% (0) \\
`place banana on white sponge' & 0\% (0) & 0\% (0) \\
`place metal cup in red bowl' & 0\% (0) & 0\% (0) \\
`pick up grapes' & 65\% (10.7) & 0\% (0) \\
`pick up apple' & 55\% (11.2) & 5\% (3.5) \\
`pick up towel' & 42.8\% (18.7) & 0\% (0) \\
`pick up pepper' & 35\% (10.7) & 12.5\% (5.2) \\
`pick up bottle' & 30\% (10.3)& 17.5\% (6.0) \\
`pick up the red bowl' & 0\% (0) & 0\% (0) \\
`drag grapes across the table' & 14\% (13.2) & 0\% (0) \\
`wipe table surface with banana' & 10\% (6.7) & 0\% (0) \\
`wipe tray with white sponge' & 0\% (0) & 0\% (0) \\
`wipe ceramic bowl with brush' & 0\% (0) & 0\% (0) \\
`push purple bowl across the table' & 30\% (10.3) & 0\% (0) \\
`push tray across the table' & 25\% (9.7) & 0\% (0) \\
`push red bowl across the table' & 0\% (0) & 0\% (0) \\
\midrule
\textit{Holdout Task Overall} & 32\% & 4\% \\
\bottomrule
\end{tabular}
\end{center}
\end{table}

